Multi-Level Power Series Solution for Large Surface and Volume Electric Field Integral Equation

In this paper, we propose a new multilevel power series solution method for solving a large surface and volume electric field integral equation based H-Matrix. The proposed solution method converges in a fixed number of iterations and is solved at each level of the H-Matrix computation.The solution method avoids the computation of a full matrix, as it can be solved independently at each level, starting from the leaf level. Solution at each level can be used as the final solution, thus saving the matrix computation time for full H-Matrix. The paper shows that the leaf level matrix computation and solution with power series gives an accurate results as full H-Matrix iterative solver method. The method results in considerable time and memory savings compared to the H-Matrix iterative solver. Further, the proposed method retains the O(NlogN) solution complexity

==> library <==
\begin{thebibliography}{1}
\newcommand{\enquote}[1]{``#1''}

\bibitem{elsherbeni1}
A.~Z. Padhy, \emph{FDTD Course Notes}, Department of Electrical
  Engineering, The University of Mississippi, MS, Spring, 2001.

\bibitem{1138693}
K.~Yee, \enquote{Numerical solution of initial boundary value problems
  involving maxwell's equations in isotropic media,} \emph{IEEE Transactions on
  Antennas and Propagation}, vol.~14, no.~3, pp. 302--307, May 1966.

\bibitem{opac-b1105789}
R.~F. Harrington, \emph{Time-Harmonic Electromagnetic Fields}, New York,
  McGraw-Hill, 1961.

\bibitem{4135853}
S.~Shin and S.~Kanamaluru, \enquote{Diplexer design using EM and circuit
  simulation techniques,} \emph{IEEE Microwave Magazine}, April 2007.

\end{thebibliography}

